Towards the Baikal Open Laboratory in Astroparticle Physics

The open science framework defined in the German-Russian Astroparticle Data Life Cycle Initiative (GRADLCI) has triggered educational and outreach activities at the Irkutsk State University (ISU), which is actively participated in the two major astroparticle facilities in the region: TAIGA observatory and Baikal-GVD neutrino telescope. We describe the ideas grew out of this unique environment and propose a new open science laboratory based on education and outreach as well as on the development and testing new methods and techniques for the multimessenger astronomy.

==> Makefile <==
FILE = open_science 

PDFLATEX = pdflatex
BIBTEX = bibtex

PDF = ${FILE}.pdf

all :	
	${PDFLATEX} ${FILE}.tex
	${BIBTEX} ${FILE}
	${PDFLATEX} ${FILE}.tex
	${PDFLATEX} ${FILE}.tex

# Various cleaning options
clean :
	/bin/rm -f  *.log *.aux *.dvi *.bbl *.blg *.bm *.toc *.out \
	*Notes.bib *.ps

